A Light in the Dark: Deep Learning Practices for Industrial Computer Vision

In recent years, large pre-trained deep neural networks (DNNs) have revolutionized the field of computer vision (CV). Although these DNNs have been shown to be very well suited for general image recognition tasks, application in industry is often precluded for three reasons: 1) large pre-trained DNNs are built on hundreds of millions of parameters, making deployment on many devices impossible, 2) the underlying dataset for pre-training consists of general objects, while industrial cases often consist of very specific objects, such as structures on solar wafers, 3) potentially biased pre-trained DNNs raise legal issues for companies. As a remedy, we study neural networks for CV that we train from scratch. For this purpose, we use a real-world case from a solar wafer manufacturer. We find that our neural networks achieve similar performances as pre-trained DNNs, even though they consist of far fewer parameters and do not rely on third-party datasets.

==> DVS Publication/sections/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Deep learning (DL) has recently received increasing attention in research and industry alike, where we can find manifold examples of successful applications like machine translation \cite{singh_machine_2017}, predictive maintenance \cite{rezaeianjouybari_deep_2020}, autonomous driving \cite{friederich2020review}, and predictive business process monitoring \cite{harl2020explainable}. Given a sufficiently large amount of training data, DL has the advantage of automatically detecting useful patterns from raw input data without the need of manually defining sophisticated features for prediction purposes \cite{kraus_deep_2020, janiesch_machine_2021}.

A field that significantly benefits from DL functionality is that of computer vision (CV). It seeks to automatically extract useful information from images to mimic human capabilities of visual perception \cite{sager_survey_2021, szeliski_computer_2010}. On this basis, time-consuming and labor-intensive tasks like the recognition, detection, localization, tracking, and counting of objects can be supported more efficiently to save resources and relieve the burden of human workers \cite{zschech_picture_2021}.

Fueled by the broad access to computing power and the availability of large image repositories, the field of CV is currently experiencing a considerable phase of scientific progress and dissemination. We can observe that a global community of developers provides user-friendly programming frameworks, shares reusable software code, and builds huge pre-trained DL models based on large-scale image repositories \cite{chollet_deep_2018, liu_deep_2020, zschech_picture_2021}. This is beneficial for many applications, since the weights of pre-trained DL models can be reused via transfer learning, which helps to build models with limited training data, save computational resources, and avoid architecture search \cite{kurkova_survey_2018}.

However, relying on pre-trained models is not always a valid option. Especially in highly regulated settings, such as manufacturing environments, pre-trained models based on public image data pose a serious security risk due to e.g. adversarial attacks \cite{heinrich_fool_2020} or induced biases \cite{janiesch_machine_2021}. Similarly, public images usually contain generic objects such as houses, cars, and animals, which rarely reflect the shapes of objects in industrial applications like technical components and surface defects \cite{zschech_mit_2020}. Beyond that, pre-trained models often consist of several million parameters \cite{heinrich_is_2019}, which limits their application on small devices with limited hardware. In an era of edge computing (i.e., computations close to the source of data, usually in real-time), these limitations become even more decisive as large models naturally lead to longer inference times. 

As a remedy, this paper studies DL-based CV models for image recognition that are created from scratch for specific business needs. Based on a real-world case from a manufacturer of solar panels, we demonstrate how our lightweight models provide competitive prediction results for the task of automated quality inspection compared to large pre-trained models. To carry out our research, we conduct a series of computational experiments and comparative evaluation studies to provide guidance for practitioners and researchers on how to successfully develop DL models from scratch.

Our paper is structured as follows: In section \ref{sec:background}, we provide an overview about the conceptual background and related work, followed by a brief description of our industrial case in section \ref{sec:case}. We then proceed to elaborate on our experimental setup in section \ref{sec:experiments} by outlining our evaluation procedures and algorithmic approaches which can basically be structured into model-centric and data-centric development steps. Subsequently, we present our results in a comprehensive manner in section \ref{sec:results}. To conclude our paper, we provide summarizing remarks and derive an outlook for future work in section \ref{sec:conclusion}.

%Even thought the application of artificial neural networks [ANNs] in the domain of artificial intelligence has already been around since 1957 with the introduction of the Rosenblatt perceptron \cite{rosenblatt1957perceptron}, the field only took off again through the huge improvements made during the ImageNet Challenge 2012\footnote{ImageNet Large Scale Visual Recognition Challenge: https://www.image-net.org/challenges/LSVRC/} by AlexNet \cite{krizhevsky2012imagenet} (a shallow convolutional neuarl network [CNN]), the outperfomance of the humans baseline during the 2015 challenge by ResNets \cite{he2016deep} (a deep CNN) and the beating of the strongest Go player in the world by AlphaGo in 2016 \cite{silver2016mastering} (a combination of ANNs and reinforcement learning techniques). 
%This development in research spawned big investments in academia, but also in business and business related research like autonomous driving \cite{friederich2020review}, automation of agriculture \cite{heinrich2019objekterkennung}, quality control \cite{trinks2019smart}, predictive/prescriptive maintenance \cite{weinzierlexploring} or process analytics \cite{harl2020explainable, stierle2021technique}. 

%The hype and influx in the use of deep learning techniques in recent years due to the availability of huge online databases and the broad access to computing power, has contributed to many advances in the fields of science, government and in business \cite{lecun2015deep}. 

%The field of computer vision, in which we are interested in this paper, has especially benefited from this influx and is experiencing a considerable phase of scientific progress and dissemination expressed by manifold activities in research and practice, which can be observed by the continuous development of advanced algorithms based on artificial neural networks \cite{bharati2020deep}. 

%Empowered by this progress, industrial applications have blossomed, like medical assistance systems (CITE), autonomous driving (CITE), and the detection of production deficiencies (CITE). 


% Was gibt es und was ist nicht so geil? -> Praxis durgehende verbreitung, Riesige Netze wurden Trainiert, immer mehr Frameworks und Standards. Bei Generischen Ojekten kann hie ralles sehr schön gelöst werden. Aber nicth in industie
% - keine Pretrained models
% - Objekte sind sehr viel spezieller als in vortrainierten Fällen - Es gibt CV, es wird viel gemacht, aber es ist meistens fast nur auf **alltagsgegenständen**
%To realize the application of computer vision systems in practice, many companies resolve to the application of huge pre-trained neural networks like VGG16 or ResNet50 from openly accessible frameworks like PyTorch\footnote{https://pytorch.org/vision/stable/models.html}. These pre-trained networks were trained on generic image data sets like ImageNet\footnote{https://www.image-net.org/}. When creating computer vision systems for the detection of generic objects, these pre-trained models are very promising to use. Problems arise when using these models, pre-trained on generic images, for very specific applications and images e.g. error-detection in solar panels. Such unknown images are much more specialized, generally very similar to each other and may consist only of simple geometrical shapes. Consequently, it is questionable, if pre-trained models achieve similar performance improvements on these specific applications over models which are trained from scratch.
% -> extrem tief, große speiter, lange inferenz
% -> shapes unterschiedlich (schon oben)
% -> Bilder nicht in eigener Kontrolle (gegen Unternehmenspolicy)

% ==> Es fehlt das wissen wie modelle von scratch trainiert werden können, ohne das sie zu komplex sind und gleichzeitig die performance haben
%Against this background, this paper looks at how computer vision models can be created from scratch for specific business needs with relative ease to guide practitioners in industry with very specialized applications. To this goal, we conduced a case study with an industry partner on the automatic classification of specific errors-types in the production of solar panels from electroluminescense images of recently produced panels.
% —> Wir wollen reflektieren: Einfach anfangen und schauen was möglich ist und dann Stückweise steigern…


% Get what is needed:
%Our examplary industrial case study is concerned with the automatic classification of errors in the production of solar panels. The task we look at is the classification of specific error-types from electroluminescense images of recently produced solar panels using CNNs, while not only differentiating looking at weather a cell is defect, but what specific defect is occurring. 
%As a further constraint, the inference time needs to be kept low to not create a bottleneck in the production process. To create a general paradigm for practice, we will structure our work with an abstraction of the CRIPS-DM approach where we only take a look at the data preparation, the modelling, the evaluation and the deployment. 
%We will propose improvements and best practices for each step to guide practitioners in implementing computer vision systems based on deep learning effectively and learn from recent advances in research that have a high impact on the performance and acceptance of systems deployed in business-critical situations. 








==> DVS Publication/sections/02_background.tex <==
\section{Conceptual Background and Related Work}
\label{sec:background}

\subsection{Computer Vision and Deep Neural Networks}
\label{sec:CV-DNN}

The field of CV is concerned with the acquisition, processing, analysis, and understanding of digital images to generate symbolic or numerical information that can be used to support automated decision-making.
Just as humans use their eyes and brains to understand the world around them, CV attempts to produce the same effect so that computers can perceive and understand an image or a sequence of images and act accordingly in each situation.
This understanding can be achieved by disentangling high-level, symbolic information from low-level image features using models built with the help of geometry, statistics, physics, and learning theory \cite{sager_survey_2021}. Driven by academic and industrial motives, grand advances have been made in several areas such as 3D model building, optical character recognition, motion capture, disease diagnostics and surveillance \cite{szeliski_computer_2010}.

Nowadays, CV tasks are increasingly performed by machine learning (ML). Of particular interest are artificial neural networks (ANNs). Inspired by information processing in biological systems, they consist of multiple interconnected neural processing units that forward signals using weights and activation functions.
ANNs learn by processing many examples and iteratively adjusting the internal weights (= trainable parameters) according to the difference between predicted outcomes and the ground truth \cite{janiesch_machine_2021, goodfellow_deep_2016}.
In advanced approaches, neural processing units are typically organised into multiple layers that can be arranged into deep network architectures. 
This gives them the capability to process spatial information in raw image data and automatically extract features that are relevant for the prediction task, which is commonly known as deep learning \cite{lecun2015deep}.

\subsection{Convolutional Neural Networks and Transfer Learning}
\label{sec:CNN-TL}

A widely used network architecture in the field of CV is that of convolutional neural networks (CNNs) \cite{lecun2015deep}. They comprise a series of stages that allow hierarchical feature learning which is a useful principle to condense low-level features into higher-level concepts. For the task of object recognition, this means that the first few layers of the network are responsible for extracting basic features in the form of edges and corners. These are then incrementally aggregated into more complex features in the last few layers resembling the actual objects of interest, such as faces, cars, or defects.
Subsequently, these auto-generated features are used for prediction purposes to recognise objects of interest \cite{goodfellow_deep_2016}.

Over time, the CV community has developed increasingly deeper CNN architectures (e.g., VGG16 \cite{simonyan}) to benefit from the functionality of hierarchical feature learning. At the same time, more advanced mechanisms like inception modules (e.g., GoogleNet \cite{szegedy_going_2015}) and residual blocks (e.g., ResNet \cite{he2016deep}) have been introduced to improve the efficiency of deep multi-layered networks.
Most of these developments are based on large scale image repositories such as ImageNet \cite{deng_imagenet_2009} or COCO \cite{fleet_microsoft_2014} that contain generic objects like cars or houses. This yields the advantage that already trained models with their adjusted weights can be reused for further recognition tasks in similar domains, which is commonly known as transfer learning \cite{pan_survey_2010, kurkova_survey_2018}. For this purpose, pre-trained models can be utilized in two different ways: 1) either as generic feature extractor where most of the weights are frozen and only the last classification layers are adjusted for the task at hand, or 2) the weights of the feature extractor and classification layers are fine-tuned on new image-label-pairs using the initial weights as starting point in case that the source domain and the target domain differ too much from each other \cite{shaha_transfer_2018}.

The key advantage of transfer learning is that it greatly simplifies the development of CV models by requiring fewer computational resources, less training time, and much smaller amounts of training data \cite{kurkova_survey_2018}.
By contrast, building DNNs from scratch usually demands well-defined development steps that cover a mixture of \textit{model-centric} design choices (e.g., choice of architecture, setting of hyperparameters, choice of regularization, etc.) vs. \textit{data-centric} design choices (e.g., data augmentation, noise removal, improvement of label quality, etc.). For this reason, transfer learning is often the preferred choice in research and industry when developing DL-based systems for CV tasks \cite{rawat2017deep}.

However, for domains with specific business needs such as given in many industrial applications, pre-trained models also bear several risks. Firstly, large pre-trained DNNs are usually built on hundreds of millions of parameters \cite{heinrich_is_2019} that prevent an deployment on many edge computing devices due to limited storage capacities and the requirement of low inference times. Secondly, industrial cases usually consist of very specific objects, such as structures on surfaces or specific technical components that heavily deviate from the shapes of general training objects of public image repositories. Lastly, using pre-trained models from foreign sources can also pose a security risk as the models can be subject to biases and adversarial attacks \cite{janiesch_machine_2021, heinrich_fool_2020}. The latter have the potential to trick and break DNNs without obvious indication which could be demonstrated, for example, with perturbations of street signs in the field of autonomous driving \cite{eykholt_robust_2018}.

%Against this background, we investigate how neural networks can achieve similar performances of competitive pre-trained DNNs, even though they consist of far fewer parameters and do not rely on third-party data sets for weight initialization.


% - kurzen Überblick geben, wo CNNs/tiefe neuronale Netze bisher eingesetzt werden - idealerweise 1-2 Review Paper (z. B. Autonomous Driving, Alltagsgegenstände, etc.)
% - auf ausgewählte Arbeiten kurz eingehen, die bereits CNN für quality inspection in industrial manufacturing verwenden
% - Quintessenz: Bisher konzentriert sich Großteil der Arbeiten auf Alltagssitutationen (Hunde, Katzen, etc.) - jedoch wenig Wissen über reale Anwendungsfälle in der Industrie und das Verhalten von tiefen neuronalen Netzen beim Umgang mit domänenspezifischen Ausprägungen (z. B. Solar Panels)

% --> deswegen will Beitrag hier Contribution leisten und mit verschiedenen Experimenten/Reflektionen anhand eines realen Cases 

%To get a better understanding of the computer vision and deep learning concepts that are applied in the rest of this paper, this section describes the fundamental ideas of machine learning, esp. deep learning in computer vision. 

 



% TODO: Introduction to Machine Learning and its sub-domains
% Machine learning is the study of how to construct computer programs that automatically improve with experience \cite{mitchell1997machine}. The field itself is roughly split into three sub-domains: supervised learning (i.e. learning from data with labels), unsupervised learning (i.e. discovering of hidden structures in data without labels) and reinforcement learning (i.e. learning by interacting with an environment) (see figure \ref{fig:sub_ml}). 
%Supervised learning is the learning from examples. The computer is presented with inputs together with their desired outputs, and the goal is to learn a general rule that maps inputs to outputs.

%Background DL & ANNs- Prototype 
%Deep learning is a sub-field of supervised machine learning. The most successful deep learning methods are deep neural networks with their wide application areas in fields like natural language processing and computer vision \cite{ongsulee2017artificial}. Artificial neural networks (ANNs), on which deep learning builds, are conceptually similar to our understanding of how to the human brain with its neuronal networks works. Biological neural networks consist of neurons that are connected by synapses \& dentrites (see figure \ref{fig:neuron}), the nodes and the connections with weights in ANNs. If the sum of excitatory signals in neurons exceeds a certain threshold, the neurons fire, just like modelled by activation functions. The goal of artificial neural networks is to replicate the way information is processed in humans by relying on nodes/neurons for analogous problem solving \cite{buduma2017fundamentals}.

% This can be cut completely, if we want to loose the background/history.
% Artificial neural networks in the broadest sense have already been around for more than 60 years with the Rosenblatt perceptron \cite{rosenblatt1957perceptron, rosenblatt1958perceptron} being one of their first representatives.
% As seen in figure \ref{fig:rosen}, a perceptron receives inputs $x = (1, x_1, x_2, \dots, x_n)$ together with a bias (a constant value that is not influenced by the inputs but represents a systematic error/displacement in combination with the input weight $w_0$). Next, the input function aggregates the inputs \textit{x} and weights $w = (w_0, w_1, \dots, w_n)$ by computing $w^T x$. Lastly, the activation function $sign$ is applied, which determines the output of the neuron depending on the inputs and the weights. In total, the perceptron computes a binary classification with $\hat{y} = sign(w^T x)$, where $\hat{y} \in \{-1, 1\}$. Typical activation functions in later works include e.g. Sigmoid, tanh, Linear, and the ReLU (Rectified Linear Unit).\\

% Nowadays, ANNs nearly always appear as multi-layer perceptrons (MLPs), where one or more hidden layers are present between the input and the output layer (see figure \ref{fig:dnn}). Each layer holds a modified representation of the data and each subsequent layer represents the data at a more abstract level. An artificial neural network is called deep if it has more than one layer but it can have an arbitrary amount of hidden layers \cite{lecun2015deep}. Here, we now speak of deep neural networks and deep learning. 
%Furthermore, it can be pointed out that in ANNs the weights are different between all nodes. This makes it possible to learn various functions and transformations during the training phase.



%\begin{figure*}[t]
%\centering
%\subfloat[Illustration of a Neuron %(adapted from \cite{neuron2021}).]{%
%  \includegraphics[width=3.5cm]{figures/neuron-structure.jpg}%
%  \label{fig:neuron}%
%}\qquad
%\subfloat[Illustration of a Perceptron (adapted from \cite{perceptron2017blog}).]{%
%  \includegraphics[width=3.5cm]{figures/rosenblatt.png}%
%  \label{fig:rosen}%
%}\qquad
%\subfloat[Illustration of a Deep %Neural Network.]{%
%  \includegraphics[width=3.5cm]{figure%s/DNN.png}%
%  \label{fig:dnn}%
%}
%\caption{TODO}
%\end{figure*}


%The PV industry is the third most used renewable energy source after hydro and wind power (Figure X). It had a record breaking year 2020 in many respects. The solar PV industry reached the biggest yearly growth in 2020 while competition and price pressures are still ubiquitous. The average module price fell by 8 \% between 2019 and 2020. Besides that, the GSR states "[...] manufactures and developers across much of the solar PV industry experienced low margins" underpinning the need for cost-effective value chains. Due to this market pressure, also a consolidating trend has been observed in the industry for a number of years. While the solar panels itself have an expected lifetime of 25 - 30 years, they get replaced much earlier due to newer technologies leading to higher efficiency and that practice ultimately leads to a growing market of second-hand panels. Finally, to tackle the challenges of climate change also political institutions, e.g. the European Commission reacts and works closely with the industry R\&D and provide investments to improve the solar technology and its production. To summarize the findings of the GSR Report, it can be stated that price pressure, the competition and the need for climate-friendly solutions all justify the need for constant optimizations and investments. Therefore, this case focuses on optimizing production, or more precisely on the automation of quality control, as part of the value chain. While \textit{automated} quality assurances are standard in many industries, e.g. software development, this might be not the case in manufacturing industries due to more complex production environments. Recent developments in the field of AI-based image recognition allows to automated processes that are still dominated by humans. As the manual check of e.g. Solar Wafers is tedious and exhausting work it is worth to automate it. 

%To be able to automate the problem, the following procedure was followed: First, images of photovoltaic wafer have to be recorded to build up a database. Therefore, a voltage is applied on the wafers to make them glow in the infrared spectral range and an IR sensitive camera takes images of that glow. This leads to the effect that faulty areas appear darker on the wafer. Next, these images are labeled according to the shown error. The wafer images and their class-label are representing the dataset that is used to train a neural network that is able to classify a wafer image into various classes. 

==> DVS Publication/sections/03_case.tex <==
\section{Case Description}
\label{sec:case}

Our case refers to the automation of quality control in the photovoltaic (PV) industry. While automated quality control is common in many industries \cite{milo_new_2015, yang_using_2020, kurdyukova_development_2020}, the PV industry is lacking behind because of complex production environments. Consequently, the PV industry often still relies on manual human controls of PV wafers which is both tedious and costly and therefore offers grand potentials for improvements via automated inspections based on DL models \cite{deitsch_segmentation_2021, zschech_mit_2020}.

For this project, we partnered with a PV wafer manufacturer. 
% Our partner recorded images of potentially damaged or malfunctioning PV wafers.
To highlight damages in wafers, voltage is applied to make the wafers glow in the infrared spectral range and an infrared sensitive camera takes images. This leads to the effect that faulty areas appear darker on the wafer. 
% Next, these images are labeled according to the shown error. The wafer images and their class-label are representing the dataset that is used to train a neural network that is able to classify a wafer image into various classes.
Next, these images are labeled according to their error to obtain our dataset that is used to train a neural network that is able to classify wafer images.

\begin{figure}[!]
    \centering
    \includegraphics[trim={0 0 0 1.3cm},clip, width=0.6\textwidth]{figures/dataset_classes.png}
    \caption{Example images for each of the eight classes.}
    \label{fig:dataset}
\end{figure}

In our case, a total of 4341 labeled images from a total of eight classes were captured by our partnering company. One class that denotes no errors, and a total of seven error-classes: low level, circle, crack, displaced, wafer on pin, splinter, and scratch. Apart from the self-explanatory classes, low level means that the glow of the wafers could not be recorded appropriately and wafer on pin means that only parts of the wafer are glowing. See Figure \ref{fig:dataset} for exemplary images of each class. 
We decided to generate three tasks from our dataset, comprising different sets of errors and, thus, varying complexity. We either used 3 classes (good, low level, circle - the classes that can be distinguished the easiest), 5 classes (good, low level, circle, crack, displaced), or all 8 classes (good, low level, circle, crack, displaced, waferonpin, splinter, scratch). The images were provided as TIFF-files with a resolution of 1024 x 1024 in 8bit grayscale. As Table \ref{tbl:descriptives} illustrates, the class distribution over the images is not balanced but differs quite heavily. 

\begin{table}[h]
\centering
\begin{tabular}{lcccc}
		    {\textbf{Class}} &
		    {\textbf{Number of}} & {\textbf{3 Classes}} & {\textbf{5 Classes}} & {\textbf{8 Classes}} \\
		    & {\textbf{observations}} \\
		\midrule
		Good & 1096 & \xmark & \xmark & \xmark \\
		Low level & 420 & \xmark & \xmark & \xmark \\
		Circle & 351 & \xmark & \xmark & \xmark \\
		Crack & 577 & & \xmark & \xmark \\
		Displaced & 993 & & \xmark & \xmark \\
		Wafer on pin & 256 & & & \xmark \\
		Splinter & 79 & & & \xmark \\
		Scratch & 569 & & & \xmark \\
		\midrule 
		$\sum$ & 4341 \\
\end{tabular}
\caption{Overview of our dataset and evaluation tasks.}
\label{tbl:descriptives}
\end{table}

%We distinguish three, five and eight classes in our evaluation. We make this distinction for three reasons: The unbalanced data distribution (which is quite common in industrial CV tasks), the weak data understanding as a non-domain expert, and to get a better overview of predictive quality of our models.

==> DVS Publication/sections/04_experiments.tex <==
\section{Experimental Setup}
\label{sec:experiments}

We conducted a series of computational experiments and compared the evaluation results systematically. Table \ref{tab:experiments} provides an overview of all experiments.

In line with our motivation to develop a lightweight yet high-performing model, we started with a simple \textit{baseline} approach in terms of a 2-layer CNN with two fully connected layers on top (ID 0). Building on this baseline, we continued with multiple experiments to increase the quality of our model, which can basically be divided into three different categories: 1) model-centric improvements, 2) data-centric improvements, and 3) a combination of both of them. 

The experiments on \textit{model-centric} improvements consider different architectural and hyperparameter-related design choices (ID 1-4). Further information is provided in Subsection \ref{sec:model-centric}. The experiments on \textit{data-centric} improvements mainly cover different data augmentation techniques (ID 5-7) and a color inversion approach (ID 8). Further details are provided in Subsection \ref{sec:data-centric}.
Since we wanted to exclude overlapping effects while also avoiding to check all combinations exhaustively due to high computational costs, the respective strands of model-centric and data-centric improvements were considered separately and \textit{combined} afterwards in case of promising effects (ID 9).

\input{tables/experiments}

In order to assess all our "from-scratch-models" against the performance of \textit{transfer learning} models, we also conducted experiments with several versions of pre-trained models. More specifically, we used a VGG16 \cite{simonyan} that is pre-trained on the widely-known ImageNet dataset \cite{deng_imagenet_2009} and can classify images into 1,000 categories of generic objects. In a first version, the pre-trained VGG16 was used as a generic \textit{feature extractor} (FE; ID 10), and in a second version, the weights were adjusted via \textit{fine-tuning} (FT; ID 11) (cf. Subsection \ref{sec:CNN-TL}). Additionally, to ensure a fair comparison, we also added the best data-centric improvement to the best performing pre-trained model (ID 12).

To provide better transparency about our overall experimental setup and the evaluation procedure, Figure \ref{fig:pipeline} summarizes our pipeline and the individual steps. As shown, we performed default data preparation steps before feeding the wafer images to the models in the corresponding experiments. These steps included resizing the images to a $256\times256$ resolution, casting the inputs to tensors, and converting the images to grayscales with one dimension. Additionally, the images for the pre-trained models were also normalized as recommended by the models. 

\begin{figure}[!]
    \centering
    \includegraphics[width=.9\textwidth]{figures/DViP_Pipeline.pdf}
    \caption{Model- and data-centric improvements procedure with common evaluation strategy.}
    \label{fig:pipeline}
\end{figure}

For our evaluation purposes, we use a stratified random split and divide our data into 60\% for training, 20\% for validation and early stopping, and 20\% for testing and the calculation of our final evaluation metrics: 1) precision, 2) recall, and 3) F1-score. Each metric is calculated with the weighted average across all classes as a common measure to assess the quality of multi-class classifiers \cite{heinrich_process_2021}. We use the F1-score as our main metric for comparisons. Additionally, we also measured the number of parameters of all trained models, the model size in megabyte (MB), and the inference times in milliseconds (ms). Across all experiments, we used the same data loading. Further, our training configurations are kept constant (cf. Appendix for details on implementation).

%In our data-centric approaches, additional transformations are used that are described in section \ref{sec:data-centric}.


\subsection{Experiments on Model-centric Improvements}
\label{sec:model-centric}
As described above, we started with a simple, yet qualitative and performant model consisting of only two convolutional layers, called \textit{BaseNet} (ID 0). This model was iteratively extended to \textit{BaseNet8} (ID 1) through the addition of more layers and a larger number of filters. On top of that, we developed \textit{BaseNet8+} (ID 2), which is the same as BaseNet8 but with changed activation functions, batch normalization and additional hyperparameters. Beyond that, we also looked into CNN architectures with more advanced processing mechanisms (cf. \ref{sec:CNN-TL}). More specifically, we developed \textit{IncNet} (ID 3), inspired by Inception Networks \cite{szegedy_going_2015}, and \textit{ResiNet} (ID 4), inspired by ResNets \cite{he2016deep}. The configurations of the individual networks are summarized in Table \ref{tab:experiments}.

% Jeweils Beschreibung + Relevante Hyperparameter oder Architecture Features - Short Description of BaseNet: 2 Conv Layers (KernelSize 5), 2 FC Layers
%The two convolutional layers include four and eight feature maps respectively with kernel size of five each with a ReLu and a MaxPooling layer with kernel size two following after each.
%The classification head includes two fully connected layers. 
%The two fully connected layer reduces the eight feature maps to the number of classes in our specific task. 
%We call this model BaseNet, evaluate it in our first experiment and use it it the following as baseline for all of our following experiments.

% Why BaseNet8 -> increase depth, bigger capacity: 8 ConvLayers (Kernel-Size 3), 2 FC Layers
%In our second experiment to improve the predictive quality of our model, we wanted to increase the capacity. We increased the amount of layers to eight and the amount feature maps to 512. This model is called BaseNet8.

% As another improvement to our BaseNet model, we replaced the ReLu activation functions with ReLu6 and added batch normalization after each convolutional layer in a third experiment. We also added a multi-step learning rate to reduce the risk of overfitting in the training phase. 
% This model is called BaseNet8+.

% Exploration: IncNet, ResiNet
%Our fourth and fifth model-centric experiment was the creation of IncNet and ResiNet. IncNet was inspired by the Inception Net architecture and incorporates different parts of the first three versions of the architecture \cite{szegedy_going_2015, szeliski_computer_2010}. 
%The architecture consists of four serial custom Inception Blocks, each consisting of a path with a $1\times1$ convolution and a $3\times3$, $5\times5$, and $9\times9$ convolution followed by another $9\times9$ convolution. ResiNet was inpired by the ResNet architecture \cite{he2016deep}. 
%It consists of four serial ResBlocks with a skip connection path and a path of two $3\times3$ convolutions.

% TransferLearning
%An often used model is the VGG16, which we also used as a representative model for this task. It is built on the well-known ImageNet data set and can classify images into 1,000 object categories. VGG16, which was proposed by \cite{simonyan}, follows a block structure where each block consists of a sequence of convolutional layers followed by a max-pooling layer. Compared to other models, the unique aspect of VGG16 is that the same kernel size (3x3) with stride 1 is applied over all convolutional layers. In the end, the model has two fully connected (FC) hidden layers and one fully connected output layer \cite{VGG16medium, VGG16}. 

%Transfer learning has become also a popular method in CV because it allows to apply complex deep CNNs in a time-saving way \citep{rawat2017deep} by using pre-trained models that were already trained on a large benchmark data set to solve a different problem. An often used model is the VGG16, which we also used as a representative model for this task. It is built on the well-known ImageNet data set and can classify images into 1,000 object categories. VGG16, which was proposed by \citet{simonyan}, follows a block structure where each block consists of a sequence of convolutional layers followed by a max-pooling layer. Compared to other models, the unique aspect of VGG16 is that the same kernel size (3x3) with stride 1 is applied over all convolutional layers. In the end, the model has two fully connected (FC) hidden layers and one fully connected output layer \citep{VGG16medium, VGG16}. 
% Considering the training architecture, we cut off the model before the last FC layer. Thus, all preceding trained layers were taken, referring to so-called frozen layers. Subsequently, just a FC layer with a number of neurons corresponding to the observed classes was added and trained anew. This minimises the computational effort in adapting the model. However, it should be noted that transfer learning involves further approaches of retraining and freezing the layers, which were not pursued further here.

% evtl gute Quelle:https://pytorch.org/tutorials/beginner/transfer_learning_tutorial.html

\subsection{Experiments on Data-centric Improvements}
\label{sec:data-centric}

In our data-centric experiments, the focus was on improving the data quality, while the underlying model remains the same. For this purpose, we used our BaseNet again for all experiments and evaluated it as described before.

% Standard augmentations
We started with some \textit{standard augmentation} (SA) techniques (ID 5) to enhance the diversity of training data across all different classes, which has already proven successful in previous studies \cite{Gu2019ImproveIC}. These augmentations include horizontal and vertical flipping, as well as 90° and 180° rotations and Gaussian Blur. In addition, we also applied normalization by calculating mean and standard deviation of the training images.

% Data Generation
Beyond that, two approaches were pursued to enhance the uneven distribution of the classes, i.e., data imbalance, by applying more specific data generation techniques. For this purpose, we chose two underrepresented classes with rather simple error structures, i.e., circles and splinters.
%Generated Images
In a first approach, an \textit{automated image composition process} (ID 6) was followed to automatically generate \textit{n} images. In short, the algorithm selects a good wafer and randomly places prior masked errors onto the good wafer image. These  errors are then positioned, resized,  blurred and rotated based on randomness to achieve a high variability among the generated images.

%DeepSMOTE
In a second experiment, we considered a more innovative generation approach called \textit{Deep Synthetic Minority Over-sampling Technique} (DeepSMOTE) \cite{dablain_deepsmote_2021} (ID 7). Based on the traditional SMOTE technique \cite{chawla_smote_2002} embedded in a deep encoder and decoder architecture, DeepSMOTE generates feature-rich images to diminish disadvantages of unbalanced classes. Over several iterations, the encoder and decoder networks were optimized until the synthetically generated images showed the necessary information density. Figure \ref{fig:Random invert} shows some development stages up to the desired level of detail.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/DeepSMOTE.jpg}
    \caption{DeepSMOTE images over several iterations.}
    \label{fig:Random invert}
\end{figure}

% Domain-specific transformations
Finally, we investigated an approach that is rather domain-specific and might not be generalizable to other domains and datasets. We tested \textit{color inversion} such that the defects on the solar panel are now represented by bright/white pixels, which correspond to high numerical values. By relying on techniques such as MaxPooling those high values are amplified.

% \subsection{Joint Consideration and Final Model}
% \label{sec:joint}

% Concluding the model- and data-centric experiments, we came up with our best custom model, namely BaseNet8+ with standard data augmentation. This model uses 80 times less parameters than VGG16 and performes competitively.

%\input{tables/small_table}
% \input{tables/big_table}


%//////Standard data preparation
% - loading, Selecting, Encoding, etc.
% - DataLoading (ImageFolder)

% - Resizing, Normalization, etc.
% - Resizing: 256
% - Normalization

% - data splitting and validation pipeleine, etc.
% - Splitting (60/20/20)

%We used our data preparation pipeline independently of the specific improvement, and the deviations from it during our different model-centric and data-centric experiments. 

%3. Select data transformations according to model 
%    basic (resize - 256, to tensor, grayscale dimension; normalization in pre-trained models) 
%    data-centric

==> DVS Publication/sections/05_results.tex <==
\section{Results}
\label{sec:results}
In this section, we present the results of our previously described experiments. We show that -- with a lightweight model -- we can achieve competitive performance compared to large pre-trained models consisting of 80$\times$ more parameters and other CNN architectures. Our main results are summarized in Table \ref{tab:5_intro}, in which we focus on the most complex case of recognizing images from eight different classes. Furthemore, we provide a complete overview of all results in Table \ref{tab:big_table} in our Appendix.

\input{tables/5_intro}

Starting from our simple BaseNet, it can be seen that the performance could be significantly elevated by our model-centric and data-centric improvements. The best performing model developed from scratch is our \textit{BaseNet8+ (+SA)} as a combination of a lightweight 8-layer CNN with improved configurations and standard data augmentations. With this combination, we could achieve a remarkable F1-score of 0.971. In contrast, the best pre-trained model achieved an F1-score of 0.99, which turned out to be \textit{VGG16-FT (+SA)} based on fine-tuning all weights and standard augmentations. Even though our best model is outperformed, it shows a huge parameter advantage by having 80$\times$ less parameters and is built without relying on training data from foreign image repositories. This also leads to the situation that our lightweight model requires far less storage capacities at 15.73 MB (52$\times$ smaller than VGG16-FT) and is extremely fast at 0.5 ms (18$\times$ faster than VGG16-FT). As alluded to earlier, these characteristics are crucial for applications in edge computing.

For further comparison, Table \ref{tab:5_intro} also contains the results of our ResiNet and IncNet models that were trained from scratch. Both approaches require a larger number of parameters, resulting in bigger model sizes and higher inference times, whereas the prediction qualities did not reach a satisfactory level. 

% the choice of the baseline model/architecture. 

%The combination of our best performing model- and data-centric improvements (BaseNet8+ (+SA)) achieved an F1-score of 0.971 compared to the combination of VGG16-FT (+SA) of 0.990 on eight classes. Even though our best model is outperformed very slightly, it has a huge parameter advantage by having 80 times less parameters and is trained without using pre-training on an unknown dataset. Table \ref{tab:5_intro} shows our best model compared to our baseline and VGG16-FT (+SA). 

% -> übersicht in der nächsten Tabelle + Gesamtübersicht im Appendix (--> APPENDIX NOCHMAL SCHAUEN OB ALLE INFOS IN TABELLE PASSEN)


\subsection{Model-Centric Improvements, Transfer Learning, and Combined Models}
\label{sec:results_detail}

To provide further insights into the findings from our experiments, we summarize the results of the model-centric improvements, the transfer learning models, and the combined approaches in a joint diagram (cf. Figure \ref{fig:model_centric_improvements}). The data-centric experiments are considered separately in Subsection \ref{sec:results_data}. Our diagram shows the prediction qualities measured via F1-score using bar graphs for 3, 5, and 8 classes, respectively, whereas a line graph indicates the number of trainable model parameters on a logarithmic scale.

\begin{figure}[h]
    \centering
    \includegraphics[width=.9\textwidth]{figures/model-centric-improvements6.pdf}
    \caption{Results of model-centric, transfer learning and combined experiments.}
    \label{fig:model_centric_improvements}
\end{figure}

Focusing on the \text{model-centric experiments} (ID 1-4), we can see a steady improvement from the BaseNet to BaseNet8 to BaseNet8+ to IncNet. ResiNet performs worse than BaseNet8+ and IncNet, while still having $2.6\times$ more parameters than BaseNet8+. ResiNet and IncNet have a significantly higher number of parameters ($36\times$ and $2.6\times$) than our BaseNet models. Due to this huge difference in number of parameters, and ResiNet performing similar to BaseNet8 and worse than BaseNet8+, as well as IncNet having the slowest inference time of all models, we decided not to pursue these two architectures any further. Instead, we added the best performing data-centric techniques in terms of standard augmentations (cf. Subsection \ref{sec:results_data}) (ID 9), which could further boost the prediction qualities by a considerable margin across all three complexity levels for our best performing model BaseNet8+ (+SA).

% transfer learning & combination
When focusing on the results from \textit{transfer learning}, we can see that all pre-trained VGG16 models (ID 10-12) generally achieve the best prediction qualities across the different complexity levels. It is notable that the VGG16-FE as generic feature extractor struggles to detect the domain-specific shapes of the different defect types on the solar panels, which is reflected by the inferior performance for five classes (0.971) and eight classes (0.939), respectively. However, once all the weights of the pre-trained model are adjusted via fine-tuning on the solar images within the VGG16-FT experiment, the model achieves outstanding results above 0.98 for all three complexity levels. Through additional standard augmentation, these results could even be raised to a performance level of over 0.99 for all classes.

Nevertheless, considering the drawbacks of these large models in terms of number of parameters, huge model sizes and high inference times, it is striking that our lightweight BaseNet8+ (+SA) model with far fewer layers and parameters comes very close to these results. As such, it can even outperform the results of VGG16-FE on five classes (0.988 vs. 0.971) and eight classes (0.971 vs. 0.939), respectively, which is also the case for our BaseNet8+ without augmentation on five classes (0.975 vs. 0.971).

%In terms of transfer learning models, BaseNet8+ (+SA) (ID 9c) outperformed VGG16-FE, but was outperformed by both VGG16-FT (ID 11c) in terms of F1-score on 8 classes. Still, VGG16-FT only had an F1-score advantage of $0.013$ while having the huge disadvantage of being $18\times$ slower and having $80\times$ more parameters.  

%It looks similar when combining VGG16-FT (+SA) (ID 12c) and comparing it to BaseNet8+ (+SA). The latter is again $18\times$ faster and has $80\times$ less parameters while only having an F1-score disadvantage of $0.019$.

\subsection{Data-centric Improvements}
\label{sec:results_data}

Considering the results of the data-centric experiments, the improvements across all implemented approaches are rather limited. Figure \ref{fig:data_centric} summarizes the results.

\begin{figure}[h]
    \centering
    \includegraphics[width=.9\textwidth]{figures/data-centric-improvements2.pdf}
    \caption{Results of data-centric experiments with fixed BaseNet model.}
    \label{fig:data_centric}
\end{figure}

It can be seen that -- compared to the baseline (ID 0) -- \textit{standard augmentations} (ID 5) led to the greatest overall improvement of approximately 0.017 (F1-score), as the transformations increase the stability of the model. Comparing the two more innovative/ sophisticated augmentation methods, both did not lead to a significant improvement. On average over the three class groupings, \textit{DeepSMOTE} (ID 6) increased the performance only by 0.001. However, it reflects characteristics of the existing data better than the \textit{generated images} which even worsened the performance by 0.003 - most probably because they introduce patterns that do not correspond to the real data. Finally, the domain-specific approach of using color inversion led to an improvement of only 0.002 on average. As all data-centric approaches, besides standard augmentation, did not show promising improvements, only standard augmentation was used for our combined experiments.


==> DVS Publication/sections/06_conclusion.tex <==
\section{Discussion and Concluding Remarks}
\label{sec:conclusion}

Industrial computer vision greatly benefits from recent developments in the field of deep neural networks. In particular, transfer learning and pre-training have allowed the usage of huge neural networks to be applied to all kinds of vision-based tasks. However, these large pre-trained DNNs are not applicable in many cases, such as in edge computing where small devices detect errors on products on the shop floor level of companies. 

To this end, we studied small, hand-crafted CNNs which are specifically powerful in their fast inference times and high accuracies. Thereby, we contribute to the field of CV, but also to the thriving field of analytics in edge computing. Exemplary, we used a case from the PV industry, in which cost-effective optimization of the value chains promises large benefits. However, our approaches are not limited to this field but can be applied to a manifold of challenges, where fast inference times on small devices are crucial.

This work is not free of limitations. In contrast to randomly exploring the search space of CNN architectures (e.g., through automated hyperparameter optimization), we decided to strategically analyse in two directions: model-centric and data-centric approaches. For the latter, we decided to try four different variations, yet, want to highlight that a manifold of other data-centric approaches are appealing. For instance, to improve the DeepSMOTE results, a further increase of the capacity of the encoder and decoder architecture could potentially improve the degree of details of generated images.  Alternatively, generative adversarial networks (GANs) \cite{goodfellow_generative_2014} might be a valuable approach to achieve a higher degree of details. Similarly, we did not evaluate all feasible combinations of our data-centric and model-centric approaches which delimits the generalizability of our findings to some extent. Furthermore, we need to diagnose our models to verify their robustness, for which we intend to use several XAI techniques \cite{barredo_arrieta_explainable_2020} in subsequent studies.

We expect that the following years will demand for more research on edge analytics. This means that more research will be needed on small, yet powerful ANNs for industry cases. This work is a first step in that direction. We exploit recent ideas in the field of CV to improve performance of specifically small models and show that our models are tough competitors for large DNNs with several hundreds of millions of parameters. In the future, we want to verify the robustness of our models in comparison to pre-trained models using XAI techniques, extend our experiments using DeepSMOTE, and want to test our approach for generalization over other datasets.

%- einige Einschränkungen - es wurden jeweils beste Ansätze ausgewählt und anschließend zum finalen modell gebracht, kann sein, dass Teilkombinationen aber bessere Ergebnisse erzielen

%- es gab noch mehr Klassen - komplexe Klassen außen vorgelassen

%- automated hyperparameter optimization rausgelassen, da es zu lange dauerte - es wird vermutet, dass hier nochmal ordentlich Performance geholt werden kann - vor allem in Custom models

%- hier Diskussion kurz eröffnen zu data-centrics vs. model-centric improvements, im Paper nur Ausblick gegeben, aber noch viel mehr möglich


%Starting from scratch might not always seem easy, but we prove that a lot of Computer Vision tasks are unnecessarily tried to be solved with way to complex pretrained models.


%DATA-Centric Ideas/Points
%- Further Improvements using DeepSmote since it relies on other AI algorithms, there is further room for improvements, e.g. understanding of use of algorithm & tunig paramater, e.g. what would happen if we use VGG architectures as encoder and decoder. My assumption would be, that the images are showing greater details than the 5-conv-layer strucure I used. Alternativly, one could also try GAN-based algorithms 
%- Generating Images with more advanced tools (not just simple Photoshop techniques). Especially the number of error per wafer (n amount of circles on a wafer) and their overall distribution (imagine a histogramm of the circle class showing, how many circle are on each wafer) across all generated images. Also, I only used 4 (circles) and ~15 masked error that can be placed on the wafer so one could maske a lot more errors to place them on the wafer to introduce even more variability. 
%- Other Data Centric approach, with more focus on data quality, e.g.  checking & cleaning labels (https://pypi.org/project/cleanlab/) since often people with less domain knowledge / label worker (which are paid) do this and error could be present..
%- another idea would be the boosting technique mentioned by @Mathias


% This is true in our specific industrial case for from scratch models, which show to be very competitive if not outperforming. 


%The PV industry is the third most used renewable energy source after hydro and wind power (Figure X). It had a record breaking year 2020 in many respects. The solar PV industry reached the biggest yearly growth in 2020 while competition and price pressures are still ubiquitous. The average module price fell by 8 \% between 2019 and 2020. Besides that, the GSR states "[...] manufactures and developers across much of the solar PV industry experienced low margins" underpinning the need for cost-effective value chains. Due to this market pressure, also a consolidating trend has been observed in the industry for a number of years. While the solar panels itself have an expected lifetime of 25 - 30 years, they get replaced much earlier due to newer technologies leading to higher efficiency and that practice ultimately leads to a growing market of second-hand panels. Finally, to tackle the challenges of climate change also political institutions, e.g. the European Commission reacts and works closely with the industry R\&D and provide investments to improve the solar technology and its production. To summarize the findings of the GSR Report, it can be stated that price pressure, the competition and the need for climate-friendly solutions all justify the need for constant optimizations and investments. Therefore, this case focuses on optimizing production, or more precisely on the automation of quality control, as part of the value chain. 

==> DVS Publication/tables/5_intro.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!]
\begin{tabular}{l|llllllll}
\textbf{ID}               & \textbf{Model}                                                                & \textbf{Precision}           & \textbf{Recall}              & \textbf{F1-score}            & \textbf{Accuracy}            & \textbf{\#Params}                 & \textbf{Size (MB)}           & \textbf{\begin{tabular}[c]{@{}l@{}}Inference\\ Time (ms)\end{tabular}} \\ \hline
0                        & BaseNet                                                                       & 0.867                        & 0.871                        & 0.864                        & 0.871                        & 7,623,832                         & 35.74               & 0.44                                                          \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{000000} 3} & {\color[HTML]{000000} IncNet}                                                 & {\color[HTML]{000000} 0.943} & {\color[HTML]{000000} 0.944} & {\color[HTML]{000000} 0.943} & {\color[HTML]{000000} 0.944} & {\color[HTML]{000000} 61,740,488} & {\color[HTML]{000000} 360.5} & {\color[HTML]{000000} 10.97}                                           \\
{\color[HTML]{000000} 4} & {\color[HTML]{000000} ResiNet}                                                & {\color[HTML]{000000} 0.905} & {\color[HTML]{000000} 0.906} & {\color[HTML]{000000} 0.904} & {\color[HTML]{000000} 0.906} & {\color[HTML]{000000} 4,453,704}  & {\color[HTML]{000000} 48.93} & {\color[HTML]{000000} 1.74}                                            \\
\textbf{9}               & \textbf{\begin{tabular}[c]{@{}l@{}}BaseNet8+ (+SA)\\ \end{tabular}} & \textbf{0.971}               & \textbf{0.971}               & \textbf{0.971}               & \textbf{0.971}               & \textbf{1,707,208}      & \textbf{15.73}               & \textbf{0.50}                                                          \\
12                       & \begin{tabular}[c]{@{}l@{}}VGG16-FT (+SA) \\\end{tabular}           & 0.990                        & 0.990                        & 0.990                        & 0.990                        & 138,357,544                       & 814.18                       & 9,13                                                                  
\end{tabular}
\caption{Results of our lightweight BaseNet8+ (+SA) compared to competitor models.}
\label{tab:5_intro}
\end{table}

==> DVS Publication/tables/big_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!]
\begin{tabular}{lll|llllll|lll}
\textbf{Approach}                                                                     & \textbf{Model}                      & \textbf{Config}                                                                                                                                                  & \textbf{ID}         & \textbf{Cl.}       & \textbf{Prec.}         & \textbf{Recall}        & \textbf{F1}            & \textbf{Acc.}          & \textbf{\#Params}                     & \textbf{\begin{tabular}[c]{@{}l@{}}Size\\ (MB)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Inf.\\ Time\\ (ms)\end{tabular}} \\ \hline
\multirow{3}{*}{\textbf{Baseline}}                                                    & \multirow{3}{*}{\textbf{BaseNet}}   & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}2-Layer, \\ Kernel-Size 5,\\ 8 Kernels\end{tabular}}}                                                         & \textbf{0a}         & \textbf{3}         & \textbf{0.955}         & \textbf{0.955}         & \textbf{0.953}         & \textbf{0.955}         & \multirow{3}{*}{\textbf{7,623,832}}   & \multirow{3}{*}{\textbf{35.74}}                              & \multirow{3}{*}{\textbf{0.44}}                                      \\
                                                                                      &                                     &                                                                                                                                                                  & \textbf{0b}         & \textbf{5}         & \textbf{0.928}         & \textbf{0.931}         & \textbf{0.927}         & \textbf{0.931}         &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & \textbf{0c}         & \textbf{8}         & \textbf{0.867}         & \textbf{0.871}         & \textbf{0.864}         & \textbf{0.871}         &                                       &                                                              &                                                                     \\ \hline
\multirow{15}{*}{\begin{tabular}[c]{@{}l@{}}Model-\\ centric\end{tabular}}            & \multirow{3}{*}{BaseNet8}           & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}8-Layer, \\ Kernel-Size 3, \\ 512 Kernels\end{tabular}}                                                               & 1a                  & 3                  & 0.988                  & 0.988                  & 0.988                  & 0.988                  & \multirow{3}{*}{1,707,208}            & \multirow{3}{*}{15.73}                                       & \multirow{3}{*}{0.50}                                               \\
                                                                                      &                                     &                                                                                                                                                                  & 1b                  & 5                  & 0.957                  & 0.957                  & 0.956                  & 0.957                  &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & 1c                  & 8                  & 0.899                  & 0.902                  & 0.899                  & 0.902                  &                                       &                                                              &                                                                     \\ \cline{2-12} 
                                                                                      & \multirow{6}{*}{BaseNet8+}          & \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}8-Layer, \\ Kernel-Size 3, \\ 512 Kernels, \& \\ Activation Layer, \\ MultiStep Scheduler, \\ BatchNorm\end{tabular}} & \multirow{2}{*}{2a} & \multirow{2}{*}{3} & \multirow{2}{*}{0.979} & \multirow{2}{*}{0.979} & \multirow{2}{*}{0.979} & \multirow{2}{*}{0.979} & \multirow{6}{*}{1,707,208}            & \multirow{6}{*}{15.73}                                       & \multirow{6}{*}{0.50}                                               \\
                                                                                      &                                     &                                                                                                                                                                  &                     &                    &                        &                        &                        &                        &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & \multirow{2}{*}{2b} & \multirow{2}{*}{5} & \multirow{2}{*}{0.975} & \multirow{2}{*}{0.975} & \multirow{2}{*}{0.975} & \multirow{2}{*}{0.975} &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  &                     &                    &                        &                        &                        &                        &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & \multirow{2}{*}{2c} & \multirow{2}{*}{8} & \multirow{2}{*}{0.937} & \multirow{2}{*}{0.937} & \multirow{2}{*}{0.937} & \multirow{2}{*}{0.937} &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  &                     &                    &                        &                        &                        &                        &                                       &                                                              &                                                                     \\ \cline{2-12} 
                                                                                      & \multirow{3}{*}{IncNet}             & \multirow{3}{*}{basic configuration}                                                                                                                             & 3a                  & 3                  & 0.987                  & 0.987                  & 0.987                  & 0.987                  & \multirow{3}{*}{61,740,488}           & \multirow{3}{*}{360.5}                                       & \multirow{3}{*}{10.97}                                              \\
                                                                                      &                                     &                                                                                                                                                                  & 3b                  & 5                  & 0.969                  & 0.969                  & 0.969                  & 0.969                  &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & 3c                  & 8                  & 0.943                  & 0.944                  & 0.943                  & 0.944                  &                                       &                                                              &                                                                     \\ \cline{2-12} 
                                                                                      & \multirow{3}{*}{ResiNet}            & \multirow{3}{*}{basic configuration}                                                                                                                             & 4a                  & 3                  & 0.966                  & 0.965                  & 0.964                  & 0.965                  & \multirow{3}{*}{4,453,704}            & \multirow{3}{*}{48.93}                                       & \multirow{3}{*}{1.74}                                               \\
                                                                                      &                                     &                                                                                                                                                                  & 4b                  & 5                  & 0.932                  & 0.935                  & 0.931                  & 0.935                  &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & 4c                  & 8                  & 0.905                  & 0.906                  & 0.904                  & 0.906                  &                                       &                                                              &                                                                     \\ \hline
\multirow{12}{*}{\begin{tabular}[c]{@{}l@{}}Data-\\ centric\end{tabular}}             & \multirow{12}{*}{BaseNet}           & \multirow{3}{*}{Standard Aug.}                                                                                                                                   & 9a                  & 3                  & 0.962                  & 0.962                  & 0.961                  & 0.962                  & \multicolumn{3}{c}{\multirow{12}{*}{see BaseNet}}                                                                                                                          \\
                                                                                      &                                     &                                                                                                                                                                  & 9b                  & 5                  & 0.942                  & 0.943                  & 0.939                  & 0.943                  & \multicolumn{3}{c}{}                                                                                                                                                       \\
                                                                                      &                                     &                                                                                                                                                                  & 9c                  & 8                  & 0.896                  & 0.897                  & 0.894                  & 0.897                  & \multicolumn{3}{c}{}                                                                                                                                                       \\ \cline{3-9}
                                                                                      &                                     & \multirow{3}{*}{DeepSMOTE}                                                                                                                                       & 6a                  & 3                  & 0.953                  & 0.954                  & 0.953                  & 0.954                  & \multicolumn{3}{c}{}                                                                                                                                                       \\
                                                                                      &                                     &                                                                                                                                                                  & 6b                  & 5                  & 0.928                  & 0.929                  & 0.928                  & 0.929                  & \multicolumn{3}{c}{}                                                                                                                                                       \\
                                                                                      &                                     &                                                                                                                                                                  & 6c                  & 8                  & 0.867                  & 0.871                  & 0.866                  & 0.871                  & \multicolumn{3}{c}{}                                                                                                                                                       \\ \cline{3-9}
                                                                                      &                                     & \multirow{3}{*}{Generated Images}                                                                                                                                & 7a                  & 3                  & 0.952                  & 0.952                  & 0.950                  & 0.952                  & \multicolumn{3}{c}{}                                                                                                                                                       \\
                                                                                      &                                     &                                                                                                                                                                  & 7b                  & 5                  & 0.919                  & 0.922                  & 0.917                  & 0.922                  & \multicolumn{3}{c}{}                                                                                                                                                       \\
                                                                                      &                                     &                                                                                                                                                                  & 7c                  & 8                  & 0.868                  & 0.873                  & 0.867                  & 0.873                  & \multicolumn{3}{c}{}                                                                                                                                                       \\ \cline{3-9}
                                                                                      &                                     & \multirow{3}{*}{Color Invert}                                                                                                                                    & 8a                  & 3                  & 0.955                  & 0.955                  & 0.954                  & 0.955                  & \multicolumn{3}{c}{}                                                                                                                                                       \\
                                                                                      &                                     &                                                                                                                                                                  & 8b                  & 5                  & 0.929                  & 0.932                  & 0.929                  & 0.932                  & \multicolumn{3}{c}{}                                                                                                                                                       \\
                                                                                      &                                     &                                                                                                                                                                  & 8c                  & 8                  & 0.871                  & 0.873                  & 0.869                  & 0.873                  & \multicolumn{3}{c}{}                                                                                                                                                       \\ \hline
\multirow{3}{*}{\textbf{Comb.}}                                                       & \multirow{3}{*}{\textbf{BaseNet8+}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}BaseNet8+ \\ (+SA)\end{tabular}}}                                                                             & \textbf{9a}         & \textbf{3}         & \textbf{0.995}         & \textbf{0.995}         & \textbf{0.995}         & \textbf{0.995}         & \multirow{3}{*}{\textbf{1,707,208}}   & \multirow{3}{*}{\textbf{15.73}}                              & \multirow{3}{*}{\textbf{0.50}}                                      \\
                                                                                      &                                     &                                                                                                                                                                  & \textbf{9b}         & \textbf{5}         & \textbf{0.988}         & \textbf{0.988}         & \textbf{0.988}         & \textbf{0.988}         &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & \textbf{9c}         & \textbf{8}         & \textbf{0.971}         & \textbf{0.971}         & \textbf{0.971}         & \textbf{0.971}         &                                       &                                                              &                                                                     \\ \hline
\multirow{9}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Transfer\\ Learning\end{tabular}}} & \multirow{3}{*}{VGG16-FE}           & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}VGG16 only for \\ feature extraction\end{tabular}}                                                                    & 10a                 & 3                  & 0.997                  & 0.997                  & 0.997                  & 0.997                  & \multirow{9}{*}{\textbf{138,357,544}} & \multirow{9}{*}{\textbf{814.18}}                             & \multirow{9}{*}{\textbf{9.13}}                                      \\
                                                                                      &                                     &                                                                                                                                                                  & 10b                 & 5                  & 0.972                  & 0.971                  & 0.971                  & 0.971                  &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & 10c                 & 8                  & 0.941                  & 0.940                  & 0.939                  & 0.940                  &                                       &                                                              &                                                                     \\ \cline{2-9}
                                                                                      & \multirow{6}{*}{\textbf{VGG16-FT}}  & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}VGG16 with all\\ weights fine-tuned\end{tabular}}                                                                      & 11a                 & 3                  & 0.997                  & 0.997                  & 0.997                  & 0.997                  &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & 11b                 & 5                  & 0.990                  & 0.990                  & 0.990                  & 0.990                  &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & 11c                 & 8                  & 0.984                  & 0.984                  & 0.984                  & 0.984                  &                                       &                                                              &                                                                     \\ \cline{3-9}
                                                                                      &                                     & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}VGG16-FT \\ (+SA)\end{tabular}}}                                                                              & \textbf{12a}        & \textbf{3}         & \textbf{1}             & \textbf{1}             & \textbf{1}             & \textbf{1}             &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & \textbf{12b}        & \textbf{5}         & \textbf{0.997}         & \textbf{0.997}         & \textbf{0.997}         & \textbf{0.997}         &                                       &                                                              &                                                                     \\
                                                                                      &                                     &                                                                                                                                                                  & \textbf{12c}        & \textbf{8}         & \textbf{0.990}         & \textbf{0.990}         & \textbf{0.990}         & \textbf{0.990}         &                                       &                                                              &                                                                    
\end{tabular}
\caption{Overall results of all experiments (baseline and best models in bold).}
\label{tab:big_table}
\end{table}

==> DVS Publication/tables/experiments.tex <==
\begin{table}[h]
\begin{tabular}{lllll}
\textbf{}                                                                    & \textbf{Model} & \textbf{ID} & \textbf{Experiment}                                                                & \textbf{Description}                                                                                                                                                                                                          \\ \hline
Baseline                                                                     & BaseNet        & 0           & Baseline                                                                           & \begin{tabular}[c]{@{}l@{}}2 conv. layers ($5\times5$ kernel) \\ + ReLu + MaxPooling ($2\times2$ kernel) \\ + 2 FC layers\end{tabular}                                                                                       \\ \hline
\begin{tabular}[c]{@{}l@{}}Model-\\ centric\end{tabular}                     & BaseNet8       & 1           & \begin{tabular}[c]{@{}l@{}}Increase capacity \\ of BaseNet\end{tabular}            & \begin{tabular}[c]{@{}l@{}}8 conv. layers ($3\times3$ kernel) + ReLu\\ + MaxPooling ($2\times2$ kernel) \\ + 2 FC layers\end{tabular}                                                                                         \\
                                                                             & BaseNet8+      & 2           & Optimize learning                                                                  & \begin{tabular}[c]{@{}l@{}}BaseNet8 + ReLu6 + batch normalization \\ + multi-step learning\end{tabular}                                                                                                                       \\
                                                                             & IncNet         & 3           & \begin{tabular}[c]{@{}l@{}}Inception-like \\network\end{tabular} & \begin{tabular}[c]{@{}l@{}}4 serial custom Inception Blocks (paths: $1\times1$ \\ convolution (1),  and $3\times3$ (2), $5\times5$ (3), \\ and $9\times9$ (4) convolution followed by \\ $9\times9$ convolution)\end{tabular} \\
                                                                             & ResiNet        & 4           & \begin{tabular}[c]{@{}l@{}}ResNet-like \\ network\end{tabular}            & \begin{tabular}[c]{@{}l@{}}4 serial ResBlocks (paths: skip connection (1), \\ and two serial $3\times3$ convolutions (2))\end{tabular}                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Data-\\ centric\end{tabular}                      & BaseNet        & 5           & \begin{tabular}[c]{@{}l@{}}Standard \\ Augmentations\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}Horizontal and vertical flipping + 90° and 180° \\ rotations + Gaussian Blur + normalization\end{tabular}                                 \\
                                                                             &                & 6           & DeepSMOTE                                                                          & Generate feature-rich images using DeepSMOTE.                                                                                                                                                                              \\
                                                                             &                & 7           & Generated Images                                                                   & \begin{tabular}[c]{@{}l@{}}Randomly places prior masked errors onto good \\ wafer image; errors are positioned, resized,  \\ blurred, and rotated randomly.\end{tabular}                                                      \\
                                                                             &                & 8           & Color Invert                                                                      & Color inversion from white to black and vice versa.                                                                                                                                                                                                   \\ \hline
Comb.                                                                        & BaseNet8+      & 9           & \begin{tabular}[c]{@{}l@{}}BaseNet8+ \\ (+SA)\end{tabular}             & \begin{tabular}[c]{@{}l@{}}Combining the best results from model-centric \\  and data-centric experiments.\end{tabular}                                                                                                            \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Transfer\\ Learning\end{tabular}} & VGG16-FE       & 10          & \begin{tabular}[c]{@{}l@{}}VGG16 for FE\end{tabular}       & Fixing all weights except for classification head.                                                                                                                                                                             \\
                                                                             & VGG16-FT       & 11          & \begin{tabular}[c]{@{}l@{}}VGG16 with FT \end{tabular}         & \begin{tabular}[c]{@{}l@{}}Unfreezing all weights and fine-tuning them for\\our case.\end{tabular}                                                                                                                           \\
                                                                             & VGG16-FT       & 12          & \begin{tabular}[c]{@{}l@{}}VGG16 with FT\\ (+SA)\end{tabular}              & \begin{tabular}[c]{@{}l@{}}Combining VGG16-FT with our standard \\ augmentations.\end{tabular}                                                                                                                               
\end{tabular}
\caption{Overview of all experiments.}
\label{tab:experiments}
\end{table}
